Fully autonomous tuning of a spin qubit

Spanning over two decades, the study of qubits in semiconductors for quantum computing has yielded significant breakthroughs. However, the development of large-scale semiconductor quantum circuits is still limited by challenges in efficiently tuning and operating these circuits. Identifying optimal operating conditions for these qubits is complex, involving the exploration of vast parameter spaces. This presents a real 'needle in the haystack' problem, which, until now, has resisted complete automation due to device variability and fabrication imperfections. In this study, we present the first fully autonomous tuning of a semiconductor qubit, from a grounded device to Rabi oscillations, a clear indication of successful qubit operation. We demonstrate this automation, achieved without human intervention, in a Ge/Si core/shell nanowire device. Our approach integrates deep learning, Bayesian optimization, and computer vision techniques. We expect this automation algorithm to apply to a wide range of semiconductor qubit devices, allowing for statistical studies of qubit quality metrics. As a demonstration of the potential of full automation, we characterise how the Rabi frequency and g-factor depend on barrier gate voltages for one of the qubits found by the algorithm. Twenty years after the initial demonstrations of spin qubit operation, this significant advancement is poised to finally catalyze the operation of large, previously unexplored quantum circuits.

==> main_content.tex <==

% \hl{TODO: 
% - look at Dom's (points, coordinates, planes, surfaces, etc) and Brandon's ('inward') papers for terminology 

% - name each stage and substage? 

% - comment on the precise things that are communicated to the next stage
% }
%The typical length of a 6-page article with 4 modest display items (figures and tables) is 2500 words (summary paragraph plus body text). The typical length of an 8-page article with 5-6 modest display items is 4300 words. A ‘modest’ display item is one that, with its legend, occupies about a quarter of a page (equivalent to ~270 words). If a composite figure (with several panels) needs to occupy at least half a page in order for all the elements to be visible, the text length may need to be reduced accordingly to accommodate such figures. Keep in mind that essential but technical details can be moved into the Methods or Supplementary Information.

%currently: ~3560 words

%Gate-defined quantum dots, with their potential to underpin scalable quantum computation and simulation, have been a focus of attention in the quantum community for over two decades~\cite{loss1998quantum, burkard2023semiconductor, vandersypen2017interfacing, hensgens2017quantum, xue2022quantum, noiri2022fast, mkadzik2022precision}. 
Recent advances underscore the potential of qubits in semiconductors for universal quantum computation~\cite{veldhorst2015two, burkard2023semiconductor, vandersypen2017interfacing, hensgens2017quantum, xue2022quantum, noiri2022fast, mkadzik2022precision, zhang2023universal}. These include the achievement of two-qubit gates showcasing fidelities that surpass thresholds essential for fault-tolerant computing~\cite{noiri2022shuttling, xue2022quantum, mills2022two}, and hot qubits that address the bottleneck of millikelvin refrigeration \cite{vandersypen2017interfacing, petit2020universal, camenzind2022hole}. Strides in wafer-scale manufacturing of these devices~\cite{neyens2023probing, zwerver2022qubits} and their efficient testing at cryogenic temperatures~\cite{de2023compact, thomas2023rapid} further highlight the rapid progress in this field.
Still, semiconductor quantum circuits are limited to at most six qubits \cite{philips2022universal} in one device. This stands in stark contrast to the potential afforded by modern semiconductor fabrication techniques, which could support the integration of millions of qubits.
%\hl{ADD: Currently just ~dozen of qubits can be operated simultaneously (quote Intel) though with modern semiconductor fabrication we could fabrication millions -> clear gap. Also, mention hot qubits?: Currently, the operational capability is limited to approximately a dozen qubits simultaneously. This stands in stark contrast to the potential afforded by modern semiconductor fabrication techniques, which could theoretically enable the integration of millions of qubits. This gap underscores a significant challenge in the field. Additionally, the emerging concept of 'hot qubits', which operate at higher temperatures than conventional cryogenic qubits, presents a promising avenue for overcoming some of the limitations of current qubit technologies.}

 One of the reasons for this contrast is that a long-standing challenge remains: the intricate tuning required to reach and maintain qubit operation. %While there have been theoretical discussions on fully automated tuning pipelines~\cite{zwolak2023colloquium, ares2021machine}, experimental demonstrations have been elusive. 
Previous works have introduced diverse approaches for automating single stages of this process, such as defining double quantum dot (DQD) confinement potentials \cite{darulova2020autonomous, moon2020machine, severin2021cross, van2022all}, navigating to specific charge transitions \cite{kalantre2019machine, zwolak2020autotuning, zwolak2021ray, nguyen2021deep, baart2016computer, czischek2021miniaturizing, durrer2020automated, lapointe2020algorithm}, fine-tuning of charge transport features~\cite{vanesbroeck2020quantum} or the inter-dot tunnel couplings~\cite{teske2019machine, vandiepen2018automated}, as well as device characterisation \cite{chatterjee2022autonomous, craig2021bridging, schuff2023identifying}. % and physical properties~\cite{botzem2018tuning}, and readout~\cite{schuff2023identifying}, 
Offering glimpses of the potential of machine learning for full qubit tuning automation, these works left the challenge unaddressed.%~\cite{craig2021bridging,matsumoto2021noise, ziegler2022toward, chatterjee2022autonomous,zwolak2023colloquium, ares2021machine}. 
%These works all targeted specific stages of the tuning process, but

Here, we present a fully autonomous tuning process, able to encode a qubit without the need for human intervention. The process of going from a fully de-energized device to the observation of Rabi oscillations, a definitive indicator of qubit functionality, %hallmark in the operation of qubits, 
usually takes human experts weeks, or even months, to complete. Our algorithm, deployed on a DQD device, % Ge/Si core/shell nanowire device, 
can complete the tuning process within three days.  %achieved Rabi oscillations in 77\% of trials, typically completing the tuning process within three days. 
 
% \hl{ADD: paragraph on results, times etc. ... The device used in this study is a Ge/Si core-shell nanowire.....The study successfully demonstrates the feasibility of fully automated tuning of spin qubits, transitioning from a grounded device state to operational control. The developed algorithm autonomously achieved Rabi oscillations in 77\% of trials, typically completing the tuning process within three days. This achievement marks a significant advancement in the field of quantum computing.

% Key to this success was the algorithm's ability to navigate through various stages of the tuning process, efficiently handling challenges and making accurate decisions. The study's approach was both robust and flexible, integrating all stages of the process and intelligently maneuvering through the parameter space. This methodology, while optimized for the specific device tested, shows potential for adaptation to similar quantum devices, though unique device types may require tailored adjustments.

% Additionally, the research offers insights into the physical characteristics of the devices. By analyzing qubit locations within the barrier gate voltage space, the team gained a deeper understanding of device physics, which can aid in accelerating the tuning of new devices with similar architecture. This understanding is further enhanced by the potential for a feedback loop between measurement and fabrication, improving both the tuning process and device fabrication.}

%Our work presents a pivotal advancement. %an experimental demonstration of a fully autonomous tuning process to encode a qubit, from a grounded device to measuring Rabi oscillations, a hallmark smoking gun in the operation of qubits. 
Our success in moving away from the manual tuning of semiconductor qubits marks a paradigm shift in quantum device scalability. Key to this success is the algorithm's ability to navigate through various stages of the tuning process, efficiently handling challenges and making accurate decisions. %, culminating our previous findings~\cite{schuff2023identifying, severin2021cross, moon2020machine}. 
Our findings, underpinned by deep learning, Bayesian optimisation, and computer vision techniques, would finally %a%dvance the accessibility and operability of 
allow for the operation and characterisation of complex, large-scale semiconductor qubit circuits. % We demonstrate the algorithm in a Ge/Si core-shell nanowire device at 1.4K. %We utilise the reliable Pauli spin blockade (PSB) observations even at relatively high temperatures~\cite{petit2020universal, petit2020high, yang2020operation, camenzind2022hole}.


\begin{figure*}[ht]
\centering
  \includegraphics[width=1\linewidth]{figures/algo_flow.pdf}

  \justifiedcaption{ \textbf{Algorithm overview.} \textbf{a,} There are four stages that the algorithm needs to successfully navigate to reach qubit operations. The goal of each stage is illustrated with a confinement potential diagram. \textbf{b,} Each stage can either be successful and produce candidates (leading to one or more branches), or unsuccessful (leading to a backtracking to the closest stage that still has candidates). The search is therefore conducted in a tree structure. Some branches of the tree might be left unexplored. This is indicated by dashed lines. Inset: Illustration of the device. Five different voltages $V_i$ can be applied to a linear confinement. \textbf{c,} A pulsing scheme can be applied with a microwave burst of length $t_\text{burst}$. The fast line is connected to plunger gate RP. \textbf{d,} Simulated measurement illustrations that mark the successful transition between stages. Starting from a stability diagram with mere DQD features (far left), the algorithm tunes parameters until promising bias triangles (middle left), triangles exhibiting PSB (middle right) and finally Rabi oscillations (far right) are obtained. The extremal points of the pulse scheme are indicated as a star and circle in the middle right illustration.}
  \label{fig:algo_flow}
\end{figure*}

\section*{Device architecture and readout technique}

We consider a common layout for a DQD device (inset of Fig.~\ref{fig:algo_flow}b). We use a Ge/Si core/shell nanowire device in which holes are confined in depletion mode \cite{carballido2023qubit}. The electrical potential is set by a number of gate electrodes. Two plunger gate electrodes predominantly shift the electrochemical potential in the left and right dots with voltages $V_\text{LP}$ and $V_\text{RP}$. The rest of the gate electrodes primarily control the barriers between the DQD and the leads as well as the inter-dot coupling. %We call the voltages that we apply to those gates  The coupling to the leads is controlled with two dedicated barrier gate electrodes with voltages $V_\text{L}$ and $V_\text{R}$. The inter-dot coupling is controlled with a barrier gate electrode with voltage $V_\text{M}$. 
One of the plunger gates is connected to a high-frequency line via a bias-tee, allowing for the application of voltage pulses and microwave bursts. 

The device can be probed by applying a bias voltage $V_\text{SD}$ to the source lead and recording the current $I_\text{SD}$ at the drain lead. %If we vary the electrochemical potential on each dot, e.g.~by varying $V_\text{LP}$ and $V_\text{RP}$, the resulting measurements are called stability diagrams. 
%Using this measurement technique instead of charge sensing techniques lowers requirements on the device and the setup but comes at the cost of comparatively slow measurements.
%The algorithm does not require the ability to measure the DQD via charge sensing or with reflectometry. This simplifies the 
The algorithm navigates to a DQD occupation that exhibits Pauli spin blockade (PSB) for spin-to-charge conversion. To achieve this, the DQD does not need to be depleted to the single hole regime. The charge occupation %$(m,n)$ 
on each dot is estimated to be in the range of several dozens \cite{froning2021strong, Froning2018, ungerer2023charge, eggli2023cryogenic}. 

The algorithm uses a two-stage pulsing protocol \cite{camenzind2022hole, maurand2016cmos, hendrickx2020single, froning2021ultrafast} which is parameterised by a microwave (MW) pulse frequency and a duration $t_\text{burst}$(Fig.~\ref{fig:algo_flow}c). This protocol allows for qubit manipulation if the spin resonance conditions are met. Details on the pulsing scheme for coherent spin control and the device are described in \ref{methods} and by Carballido \textit{et al.}~\cite{carballido2023qubit}. %The qubit is initialized in a spin-blockaded, effective triplet state with one charge on each quantum dot. % by employing a specific plunger gate voltages $V_\text{RP}$. 
%After a short waiting period, the system is pulsed into Coulomb blockade with a square pulse of height $\Delta V_\text{RP}$. While in Coulomb blockade, a microwave (MW) pulse of duration $t_\text{burst}$ is applied. Pulsing back to the initial point produces a current $I$ that is proportional to the likelihood of a singlet configuration after coherent manipulation due to spin-to-charge conversion via Pauli spin blockade (PSB). 
 
%We use a Ge/Si core-shell nanowire device in which holes are confined in depletion mode. The device is described in more detail in \ref{methods} and by Carballido \textit{et al.}~\cite{carballido2023qubit}.


%The device consists of a Ge/Si core/shell nanowire (NW) lying on top of nine bottom gates. By applying positive voltages to the first five bottom gates from the left, an intrinsic hole gas inside the NW is depleted to form a hole DQD. This DQD has a net-effective hole occupation (m,n) on the left and right dot, with the total hole occupation estimated to be in the range of several dozen, as described in detail in references [36, Froning2018, Froning2021a, Ungerer2023, Eggli2023]. 
%The Ge/Si core-shell nanowire device used in this study is described in detail in \cite{carballido2023qubit}.


%We assume a common layout for a double quantum dot (DQD) device with an initial quasi-1D confinement, see Fig.~\ref{fig:algo_flow} for an illustration of the device. Two plunger gate electrodes control the electrochemical potential of each dot with voltages $V_\text{LP}$ and $V_\text{RP}$. The coupling to the leads is controlled with two dedicated barrier gate electrodes with voltages $V_\text{L}$ and $V_\text{R}$. The inter-dot coupling is controlled with a barrier gate electrode with voltage $V_\text{M}$. The current across the double quantum dot is measured with an applied bias voltage $V_\text{SD}$. One of the plunger gates is connected to a fast line that allows microwave pulses to manipulate the qubit. Slower pulses on the same line can be used to quickly bring the device into Coulomb blockade, where qubit manipulation can be performed, and back again to the readout point. Here we use Pauli spin blockade (PSB) for spin-to-charge conversion (PSB)~\cite{hanson2007spins} and measure by comparing the signals with and without a driving pulse using a lock-in amplifier. %To amplify the measurements, we use lock in measurements of the current that compare the pulsed and unpulsed current. 
%The Ge/Si core-shell nanowire device used in this study is described in detail in \cite{carballido2023qubit}.

%Our algorithm is able to tune a qubit within 36h. We are mostly limited by the integration time of direct current measurements and the time needed to set voltage in the digital-to-analogue converter. The starting point of the algorithm is safe ranges that are determined via leak tests of the gates. We further require to set some hyperparameters that are derived from the expected size of features, e.g.~bias triangles. 

% \section{Device and overview}



% Todo: introduce basics: barrier, plungers, measurement technique, stability diagrams, 



\begin{figure*}
\centering
  \includegraphics[width=1\linewidth]{figures/algo_details.pdf}

  \justifiedcaption{ \textbf{Summary of each stage.} %Each stage includes several steps with various search and signal processing algorithms. 
  \textbf{a,} Stage 1: Definition of a DQD potential. 
  \textbf{a-\textit{i}} Current measurements along random directions in gate voltage space to determine the points at which conducting and non-conducting regions meet, so-called pinch-off points.
\textbf{a-\textit{ii}} Gaussian processes model the hypersurface after collecting sufficient pinch-off points.
\textbf{a-\textit{iii}} A neural network confirms the presence of a DQD analysing the aquired stability diagrams.
  %The first stage defines a hypersurface that separates conducting regions from isolating regions. This is done by taking current measurements along randomly selected directions in the barrier voltage space, see \textbf{a-i}. When a pre-defined number of pinch-off points are collected, we use a Gaussian process to model the hypersurface, see \textbf{a-ii}. Pinch-off measurements of the three individual barrier gates define a search region at the corner of the hypersurface. A neural network finally confirms the existence of a DQD using a stability diagram see \textbf{a-iii}. 
  \textbf{b,} Stage 2: Optimisation of bias triangle features.
  %Given the extent from the previous stage, an optimisation of the bias triangles in the stability diagram is performed. 
  \textbf{b-\textit{i}} Analysis of stability diagrams, segregating individual transitions and averaging them along segments orthogonal to the detuning axes.
  %shows the basis of a the optimisation: stability diagrams are taken, split intro the individual transitions and each transition is projected onto its detuning axis. 
  \textbf{b-\textit{ii}} Distribution of optimisation scores and averages of bias triangles along segments orthogonal to their detuning axes. We aim to increase the singlet-triplet energy splitting via a proxy score that measures the dip of current between the baselines and the rest of the triangles.
  \textbf{b-\textit{iii}} Identification of plunger voltage windows unaffected by charge switches aided by neural networks.
  %shows two such projection and an example distribution of the scores. The score favors a separation of the base line of the bias triangles from the tips. The stage defines a window for the plunger voltages that are not affected by charge switches, visualised in \textbf{b-iii}. 
  \textbf{c,} Stage 3: Finding PSB
  \textbf{c-\textit{i}} Initial low-resolution, wide-range detection of PSB using neural networks.
  \textbf{c-\textit{ii}} Detailed high-resolution scans employing segmentation algorithms.
  \textbf{c-\textit{iii}} Bias triangles that show signatures of PSB and can be used to optimise readout.
  %The third stage tests each transition in the given window for Pauli spin blockade in, first in a low-res wide-shot using neural networks (\textbf{c-i}), then in a high res scan using a segmentation algorithm (\textbf{c-ii}). The segmentation is also used downstream to define suitable search regions for readout spots. The outcome of this stage is candidates with PSB that potentially host qubits. For a typical measurement of such a stage, see \textbf{c-iii}. 
  \textbf{d,} Stage 4: Readout spot identification within a promising transition
  \textbf{d-\textit{i}} Acquisition of stability diagrams pulsing gate RP to locate the readout region (indicated by a white dashed box).
  \textbf{d-\textit{ii}} Entropy-based scoring of magnetic field traces within the readout region, optimized through Bayesian methods.
  \textbf{d-\textit{iii}} Rabi oscillations for different magnetic fields around the resonance condition to confirm qubit operation. The measurements marked with $I_\text{LI}$ were amplified with a lock-in amplifier, see \ref{methods} for details.
  %Within a promising transition, a readout spot is searched for using traces over the magnetic field. First, the stability diagram with pulsing needs to be taken and the readout region detected, see white dashed box in \textbf{d-i}. Then, traces within that box are taken and scores, see \textbf{d-ii} The traces are scored on their entropy and optimised via Bayesian optimisation. Finally, various qubit measurements are taken, including Rabi chevrons, see \textbf{d-iii}.
  }
  \label{fig:algo_illustration}
\end{figure*}

\section*{The algorithm}

The autonomous tuning algorithm is structured into four main stages. Starting from a completely de-energized device, i.e.~with all gate voltages set to 0, the first two stages define the DQD potential by tuning the inter-dot barrier and the reservoir coupling. The third stage narrows the search space by looking for distinct signatures of PSB, an initialisation and readout requirement. The last stage fine tunes the plunger voltages and finds the frequency and duration of a microwave pulse needed to drive the qubit. The effect of each stage on the DQD confinement potential is illustrated in Fig.~\ref{fig:algo_flow}a. Measurement illustrations exemplifying those taken by the algorithm are shown in Fig.~\ref{fig:algo_flow}d.


As a result of the algorithm design a search tree emerges, as shown in Fig.~\ref{fig:algo_flow}b. Once a stage is successfully completed, a list of candidates is generated. A candidate consists of all information needed for the next stage to investigate it, usually containing locations or ranges of gate voltages, or information on the suspected $g$-factor and Rabi frequency $f_\text{Rabi}$. The candidates are ordered by a dedicated score in each stage and a single candidate is passed on to the next stage. %Thus, the algorithm prioritizes depth over breadth whenever a stage was completed successfully. 
If a stage is unsuccessful, the algorithm backtracks to the previous stage and investigates the next candidate in that stage's list of candidates. This process dynamically creates a search tree. If a different branch has proven to lead to a qubit, some branches of the tree may be left unexplored. These are indicated by dashed lines in the tree in Fig.~\ref{fig:algo_flow}. 

 We describe each stage in this section. Details on the stage structures, substages, and composition of candidates for each stage can be found in \ref{methods} and the Supplementary Material.

%The search tree with varying depth as well as unexplored but possible branches, as shown in the center of Fig.~\ref{fig:algo_flow}. 



\subsection*{Stage 1: Define DQD}

The first stage identifies the gate voltage settings that define the DQD confinement potential. It determines a lower and upper limit for each barrier gate voltage, which is used in subsequent stages.


Building upon the methodologies of Moon \textit{et al}.~\cite{moon2020machine} and Severin \textit{et al}.~\cite{severin2021cross}, a hypersurface model is created to distinguish between conducting and non-conducting regions within the three-dimensional barrier gate voltage space.
The algorithm takes current measurements along random directions within this space (Fig.~\ref{fig:algo_illustration} a-\textit{i}), and models the hypersurface with a Gaussian process, as depicted in Fig.~\ref{fig:algo_illustration} a-\textit{ii}. We expect a DQD potential forming near a corner of the hypersurface in the first octant. To pinpoint this corner, three specific current measurements are conducted using only one of the gate electrodes at a time. The resulting coordinates are then projected onto the model of the hypersurface, setting the lower bounds of the region where DQDs are likely to be found. The upper bounds of the region are given by the coordinates of the single gate pinch-off voltages, i.e.~when the current drops to a value that is indistinguishable from the noise floor. The resulting box is labelled as `DQD search region' in Fig.~\ref{fig:algo_illustration} a-\textit{ii}.


A methodical search within this box is conducted by the algorithm. The algorithm samples locations in the DQD search region and investigates them, starting from the point nearest to the projected corner and progressing to higher gate voltages. At each location a one-dimensional trace of the plunger gate voltages is taken and checked for Coulomb peaks, a signature for quantised charge transport and a first requirement for a DQD. % using the classifier developed by Severin \textit{et al}.~\cite{severin2021cross}. 
If Coulomb peaks are found, a measurement varying both plunger gate voltages, a so-called stability diagram, is acquired and analyzed via a neural network for DQD characteristics; see Fig.~\ref{fig:algo_illustration} a-\textit{iii} for a stability diagram that shows the desired features. %This analysis employs a neural network, which has been trained on a combination of data and labels from the studies by Moon \textit{et al}.~\cite{moon2020machine} and Severin \textit{et al}.~\cite{severin2021cross}, as well as additional data sourced from a nanowire device different from the one currently in use. 
Successful identification of DQD features at a location in gate voltage space establishes it as a lower limit for the subsequent search. 


%We sample quasi-random points inside the corner box and investigate each point, starting from the one closest to the original corner. At each point, we  take a one dimensional trace and use the classifier developed in \cite{severin2021cross} to classify for Coulomb peaks. If this test is passed, a 2D stability diagram is taken and classified for double dot features. We use a neural network trained on data and labels from \cite{moon2020machine, severin2021cross} and added data from a nanowire device different from the one used here. Once this test is passed, we use the location as a lower bound. Both bounds are passed to the next stage.



%tasked with defining a DQD potential. This requires the detection of double dot features in charge transport measurements with varying potential in each dot, so-called stability diagrams. 
%We vary the plunger voltages and measure the current across the DQD, illustrated in Fig.~\ref{fig:algo_flow}.
% Further details on each stage are described in the next section.




\subsection*{Stage 2: Tune barriers}

The goal in the second stage is to adjust the tunnel barriers to enhance the %features of the bias triangles, specifically aiming for a distinct separation between the baseline and the rest of the triangle. This is critical because it signifies sufficient 
singlet-triplet energy splitting, an important requirement for qubit operation. Additionally, this stage needs to avoid regions of gate voltage space with following characteristics: regions with high currents above a generous threshold; regions that are susceptible to charge switch noise; regions that show co-tunneling lines.

%The second stage focuses on further tuning the barriers such that the bias triangle show promising features, i.e.~a good separation of the base line from the rest of the bias triangles. This indicates energy splittings that are high enough to enable qubits. 

Within the gate voltage bounds established in the first stage, Bayesian optimisation is employed to search gate voltage combinations. The figure of merit for this optimisation is based on the degree to which it reduces current between the triangle baseline and excited states, compared to the current throughout the rest of the bias triangles. This acts as an easy-to-compute proxy score of the singlet-triplet energy splitting. After Bayesian optimisation suggests a voltage setting, a stability diagram is measured (Fig.~\ref{fig:algo_illustration} b-\textit{i}). We first use a segmentation algorithm \cite{kotzagiannidis2023bias} to find the outlines of individual pairs of bias triangles. The score is then computed using averages of the stability diagram along the common baseline, as illustrated in Fig.~\ref{fig:algo_illustration} b-\textit{ii}. A neural network identifies bias triangles that are impacted by charge switches. Charge switches distort the stability diagrams and make the area unsuitable for qubit operation; see the hatched area in Fig.~\ref{fig:algo_illustration}b-\textit{iii} or Extended Data Fig.~\ref{fig:switch_illustration} for examples. These bias triangles are excluded from the optimisation. The gate voltage regions explored by the optimisation are shown in Fig.~\ref{fig:algo_illustration} b-\textit{ii}.   % This neural network is trained on data collected from the same device through an automated tuning process.

A significant challenge of this stage is the need for numerous stability diagrams, which are time-intensive to measure. To address this, we implement an adaptive, efficient measurement algorithm designed to specifically focus on gate voltage regions where bias triangles are present, see Supplementary Material for details. Employing this method cuts down the measurement time by approximately two-thirds. The optimisation is performed using these efficient measurements.

As a final step, stability diagrams without the efficient measurement algorithm are taken in the most promising regions. This is done to ensure there are no charge switches, because the previous step ranked each location by the highest score of a bias triangle at that location. Therefore, some stability diagrams may have regions affected by charge switches. Bounding boxes are then created in the plunger voltage space, encompassing primarily stable bias triangles with current below the previously mentioned threshold (Fig.~\ref{fig:algo_illustration} b-\textit{iii}). These triangles are each evaluated and scored, and the bounding boxes are ranked based on the highest score they contain.

The algorithm has up to this point only used a positive bias voltage. This stage proposes both positive and negative bias voltages for each candidate it creates. The gate voltage coordinates including the bias voltage are passed on to the subsequent stage. 

%Within the bounds given by the previous stage, a Bayesian optimisation is performed. The optimisation score hinges on the suppression of current in the valley between base line and excited states compared to the current in the rest of the bias triangles. With the aid of neural networks, unstable bias triangles that are affected by charge switches are detected and discarded. %The network was trained on data from the same device that can be gathered using the automated tuning pipeline. 
%This stage requires many large stability diagrams which are expensive in time to take. To combat this, we employ an adaptive efficient measurement algorithm that aims to only take data where there are bias triangles. As a last step, full 2D measurements (i.e.~without the efficient measurement algorithm) of the best regions are taken and checked for switches. Bounding boxes in the plunger voltages space are drawn to included mostly non-switchy bias triangles of low current. The triangles in the boxes are scored and the boxes are ranked by the highest score within their bounds. The barrier voltages and bounding boxes for plunger voltages are passed to the next stage.

\subsection*{Stage 3: Find PSB}

In this stage, our algorithm searches for charge transitions exhibiting PSB, a necessary condition for qubit initialisation and readout in this setup. A candidate has to pass three different classifiers to be judged as exhibiting PSB. This is necessary to avoid false positives entering the time-intensive last stage.

We begin with low-resolution stability diagrams of bias triangle candidates, both with $B=0$ T and $B=0.1$ T. In these devices, PSB is expressesd as a suppressed baseline of the bias triangles in low magnetic field compared to high magnetic fields (Fig.~\ref{fig:algo_illustration} c-\textit{iii}).

%In the third stage the spotlight is on identifying Pauli Spin Blockade (PSB). 
%First, low resolution measurements of the proposed candidate are taken with and without magnetic field. In the given system, PSB should be visible as a missing base line in a measurement with low magnetic field compared to high magnetic field, see Fig.~\ref{fig:algo_illustration} c-iii for an example. 

We use a routine based on the auto-correlation of the stability diagram to pinpoint bias triangle locations, see \ref{methods} for details. % the auto-correlation of these measurements to pinpoint bias triangle locations, utilizing the underlying periodicity of measurements with multiple bias triangles. 
The identified triangles are then analyzed using a neural network%, as detailed by Schuff \textit{et al.}
~\cite{schuff2023identifying}(Fig.~\ref{fig:algo_illustration} c-\textit{i}). Subsequently, the algorithm measures a stability diagram to precisely delineate the bias triangle, followed by high-resolution stability diagrams with $B=0$ T and $B=0.1$~T.

The algorithm invokes a routine to segment the bias triangles \cite{kotzagiannidis2023bias}, illustrated in Fig.~\ref{fig:algo_illustration} c-\textit{ii}. A further PSB classification based on the segmentation is performed. The routine from \cite{kotzagiannidis2023bias} defines the direction in plunger voltage space that controls the detuning $\varepsilon$ of the dot energies, known as the detuning axis of the bias triangles. Scanning along this line with varying magnetic fields, we expect to observe a current drop at the baseline at zero magnetic field, which another classifier detects.
Upon meeting all criteria, the gate voltage coordinates are forwarded to the next stage.

%We use information from the auto-correlation of the measurement to identify bias triangle locations. The bias triangles are then classified using the neural network introduced in \cite{schuff2023identifying}. This is visualised in Fig.~\ref{fig:algo_illustration} c-i. %We retrained the neural network with new automatically acquired data from this device to improve performance. 
%After this, a re-centering scan that finds the exact outline of the bias triangle is taken and then high resolution measurements of the bias triangle at low and high magnetic fields. We use a second classifier that segments the bias triangles to classify for Pauli spin blockade again \cite{kotzagiannidis2023bias}, see Fig.~\ref{fig:algo_illustration} c-ii for an illustrative measurement and a segmentation outline. 

%Finally, the algorithm from \cite{kotzagiannidis2023bias} also provides the definition of the detuning line of the bias triangles, which we use to scan along the detuning line with varying the magnetic field. We expect to see a drop in current at the base line which another classifier looks for. Once all criteria are met, the gate voltage parameters are passed to the next stage.


\begin{figure*}[htbp]
\centering
  \includegraphics[width=1\linewidth]{figures/tuning_times_locations_v2.pdf}

  \justifiedcaption{ \textbf{Benchmarking.} \textbf{a,} The duration of each stage for ten successful runs is shown, sorted by the total time taken to tune a qubit in operation. In black: the three runs that did not lead to a qubit. \textbf{b,} Locations in the barrier voltage space (as a fraction of the individual pinch-off voltage) is shown. In some locations, no PSB was identified. The qubit locations are a subset of locations that exhibit PSB. \textbf{c,} Examples of transitions from two different runs, showing the associated bias triangles (upper row) and Rabi chevrons (lower row). \textbf{d,} Characterisation. Varying the barrier gate voltages, we can build a map of $f_\text{Rabi}$ (top row) and the $g$-factor (bottom row) of one of the found qubits (marked with arrows in b) using automated measurements. For illustrative purposes we show slices of a Gaussian Process model that was fitted to the data.}
  \label{fig:results}
\end{figure*}
\subsection*{Stage 4: Find readout}

The final stage of the process is dedicated to finding an operating point for qubit readout and manipulation. %within the bias triangles, essential for effectively driving a qubit. 
This stage not only identifies a suitable location in plunger voltage space but also determines the optimal driving frequency and duration of the pulse.


Based on the segmentation from the previous stage, a predicted readout gate voltage region within the bias triangle is defined (Fig.~\ref{fig:algo_illustration} d-\textit{i}). The algorithm optimizes across the four-dimensional space of the two plunger gate voltages, the driving frequencies and pulse durations. It samples a point within this space and then measures the current as a function of the magnetic field (Fig.~\ref{fig:algo_illustration} d-\textit{ii}). The optimisation's goal is to identify a current peak in these scans, indicative of the qubit's resonance condition (Fig.~\ref{fig:algo_illustration} d-\textit{ii}, lower right plot). This is achieved by evaluating the entropy of current traces; traces exhibiting a peak correspond to lower entropy values, see \ref{methods} for details. 

%In this phase, the focus is on discerning the Electron Dipole Spin Resonance (EDSR) signal within a lockin-amplified current. 
%The same segmentation technique as used in the previous stage is employed to delineate an expected readout area within the bias triangle, see Fig.~\ref{fig:algo_illustration} d-i. The algorithm optimises over the spaces spanned by the coordinates of this box, and  a range of driving frequencies and durations. A point in this 4-dimensional space is sampled and then the algorithm scans over the magnetic field. The objective of the optimisation is to find a peak in these scans which indicate the qubit frequency, see Fig.~\ref{fig:algo_illustration} d-ii, lower right plot. This is done via a score that computes the entropy of the traces. Traces with a peak have a low entropy.
%to find an \hl{To identify the most promising regions within this area, Bayesian optimization is applied across a range of frequencies and burst durations. This optimization involves scanning against the magnetic field while recording both the in-phase and out-of-phase components of the lockin signal. The key objective of the Bayesian optimization is to locate areas of low entropy, which typically correspond to regions with a distinct peak indicating the qubit's frequency, see Fig.~\ref{fig:algo_illustration} d-ii

Bayesian optimisation then proposes potential candidates for further analysis. These candidates are filtered based on the presence of one or two peaks (corresponding to the number of qubits addressed), as determined by a simple peak-finding algorithm \cite{2020SciPy-NMeth}. Noisy measurements might also show peaks. Therefore, a follow-up step involves retaking the measurement to confirm the presence of a peak.% and to rule out the possibility of it being mere noise.

Once a candidate is verified, several measurements are taken by the algorithm to establish the qubit's operational functionality. These include a spectroscopy measurement, a Rabi chevron experiment (Fig.~\ref{fig:algo_illustration} d-\textit{iii}), and repeated high resolution Rabi oscillations at the Larmor frequency.

%is carried out, measuring the current while varying the driving frequency against magnetic field. Subsequently, a Rabi chevron experiment is conducted to further characterise the qubit properties, see Fig.~\ref{fig:algo_illustration} d-iii.

%The insights gained from this analysis inform the last step - measuring repeated one-dimensional Rabi oscillations at the identified frequency of the qubit.% This comprehensive approach ensures that the operating point, frequency, and duration are optimally set for efficient qubit operation.

%The fourth stage is all about discerning the Electron Dipole Spin Resonance (EDSR) signal within a lockin-amplified current. 
%A segmentation technique creates an outline within the bias triangle, marking the expected readout area. A Bayesian optimisation is performed within this box and for a range of frequencies and burst times by scanning against the magnetic field and recording the in-phase and out-of-phase components of the lockin signal. The Bayesian optimisation searches for low entropy locations. This leads to regions with a pronounced peak where the frequency of the qubit is found. The Bayesian optimiser proposes candidates to the next stage if they have 1 or 2 peaks judged by a simple peak finding algorithm (cite scipy). As a next step, a check is done by re-taking the lockin measurement and verifying that a peak is actually present and this was not noise. If this check is passed a spectroscopy measurement is performed of frequency vs. magnetic field. Then, the expected magnetic field at a certain frequency is computed and Rabi chevron is done. A simple analysis of of the frequency informs the next step, which is to take repeated 1D Rabi oscillations at the frequency of the qubit.



% \section*{Inner workings of the stages}





% More details on each stage can be found in section \ref{methods}.
\subsection*{Hyperparameters}
Each stage requires a set of hyperparameters. They control various aspects of the measurements such as: resolution and safe gate voltage ranges for stability diagrams; aspects of the signal processing algorithms such as the required prominence of peaks; and steering parameters such as the number of candidates that a stage can suggest. The measurement aspects can be derived from some weak prior knowledge about device such as the magnitude of lever arms which informs the resolution of stability diagrams. We also assume a $g$-factor larger than 0.5 (limiting $B$ and $f_\text{MW}$) and a $f_\text{Rabi}$ between $30$ MHz and $250$ MHz (limiting $t_\text{burst}$). The requirements on the prior knowledge can be easily softened by widening the search space.

The set of hyperparameters influences the length of the runs and the way the algorithm manages trade-offs between exploration and exploitation. Regardless of the hyperparameters, the algorithm will always terminate once all candidates of each stage have been exhausted.

The choice of hyperparameter was made during development and  not optimised for total run time or efficiency. %Minor alterations to them are unlikely to have a large impact on performance.
We provide a full list of all hyperparameters in the Supplementary Material.

\subsection*{Characterisation}

After a qubit has been found, we may choose to study the qubit further. Routines from Stages 3 and 4 enable the tracking of a known readout spot and the resonance condition in gate voltage space. This allows for the recording the dependency of qubit metrics as we change the confinement potential. We provide details of this characterisation algorithm in \ref{methods}.

\section*{Results}


%\subsection*{Experiment Setup and Main Results}

%The starting point of the algorithm is a completely de-energized device. %, i.e.~with all gate voltages set to 0V, 
We fixed the hyperparameters and gathered 13 runs.
%and using the same set of hyperparameters 13 times. 
Rabi oscillations were found in ten of those runs. 
In successful runs, the time spent in each stage varied (Fig.~\ref{fig:results}a).
% , with the mean (median) times being 1.2 h (1.2 h), 14.5 h (14.6 h), 11.1 h (10.2 h), and 11.6 h (6.3 h), respectively.
% All run times are shown in Fig.~\ref{fig:results}a. The 
total time required ranged from 22 to 80 hours, with a mean of 38 hours (median 34 hours) (Table \ref{tab:metrics}). Each stage relies on the exploration and accuracy of the previous stage. The variation in the time required in each stage gets progressively larger. % As each stage might make small mistakes, the compounded mistakes express as larger times. 
Almost all time is spent on measuring the device, not on the decision algorithms. This is due to the measurement of current through the DQD which requires long integration times. A setup that allows for fast measurements via, e.g.~radiofrequency reflectometry could be tuned orders of magnitudes faster.

\begin{table}[!ht]
    \centering
    \begin{tabular}{r||l|l|l|l|l|l|l|l|l|l}
    \toprule
        Run \# & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ \midrule \midrule
        Time & 22.8 & 24.5 & 28.5 & 32.0 & 33.3 & 34.4 & 34.5 & 37.8 & 56.5 & 79.2\\
        (h)  & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~   \\ \midrule
        $f_\text{Rabi}$& 31 &	97&	109&	47&	51&	90&	56&	115&	49&	63 \\ 
        (MHz) & \tiny$\pm$1 & \tiny$\pm$2 & \tiny$\pm$1 & \tiny$\pm$1 & \tiny$\pm$1 & \tiny$\pm$1 & \tiny$\pm$1 & \tiny$\pm$3 & \tiny$\pm$1 & \tiny$\pm$1 \\ 
        $g$ & 1.52&	0.72&	0.70&	2.20&	2.74&	0.73&	2.31&	0.67&	2.12&	0.74 \\
        &   \tiny $\pm$0.07&  \tiny$\pm$0.05&  \tiny$\pm$0.05&  \tiny$\pm$0.12&  \tiny$\pm$0.22&  \tiny$\pm$0.04&  \tiny$\pm$0.14&  \tiny$\pm$0.08&  \tiny$\pm$0.14&  \tiny$\pm$0.03\\\midrule
        $V_\text{L}$ (V) & 1.34 & 1.34 & 1.34 & 1.37 & 1.36 & 1.35 & 1.35 & 1.32 & 1.35 & 1.38 \\ 
        $V_\text{M}$ (V) & 0.69 & 0.81 & 0.79 & 0.80 & 0.69 & 0.78 & 0.79 & 0.77 & 0.65 & 0.71 \\ 
        $V_\text{R}$ (V) & 0.91 & 1.02 & 0.95 & 1.01 & 1.04 & 0.94 & 0.95 & 0.89 & 1.00 & 1.02 \\ \bottomrule
    \end{tabular}
    \justifiedtablecaption{\textbf{Metrics of successful runs.} For each qubit found, we show the total time it took, the Rabi frequency $f_\text{Rabi}$, the $g$-factor, and the settings for the barrier gates $V_\text{L}$, $V_\text{M}$ and $V_\text{R}$. The errors of $f_\text{Rabi}$ are estimated from the fit uncertainty and the errors of $g$ are calculated from the width of the resonance peak.}
    \label{tab:metrics}
\end{table}

The three failed runs terminated after their exploration on a similar timescale to the longest successful runs. They took between 56.0 h and 94.9 h to complete and are shown in black in Fig.~\ref{fig:results}a. The runs found transitions that showed Pauli spin blockade but the algorithm was not able to find Rabi oscillations, possibly due to unfortunate settings of the tunnel barrier strengths in Stage 2. 
%The large variations in the last two stages are due to transitions that were classified as having PSB (creating candidates to investigate on the last stage) but with no readout spot being found. If the first candidate that is found is also turned into a qubit, the last two stages were very short.

The qubit locations in gate voltage space in terms of the three barrier gate voltages are depicted in Fig.~\ref{fig:results}b. For comparability, we normalise each voltage by the voltage at which each barrier gate electrode pinches off the current individually. At each point, Stage 2 (Tune barriers) passed a candidate for further analysis (solid dots). In some cases, PSB was detected (dashed circles), passing Stage 3, and a subset of these also yielded a qubit (solid circles), successfully completing Stage 4.

Fig.~\ref{fig:results}c presents examples from two runs, showing the transitions found and Rabi chevron measurements. The discovery of qubits in both bias directions evidences the algorithm's adaptability and its non-specificity to certain transitions. Both Rabi chevrons were obtained using the same given driving power and driving frequency, but varied in magnetic fields and Rabi frequencies, highlighting the algorithm's generalization capability. All depicted measurements were autonomously executed by the algorithm, accounting for the non-centered chevron measurements.

%\subsection*{Insights from Experiments}

Analyzing the locations in gate voltage space where qubits were found provides insight into the device physics (Table \ref{tab:metrics}). By fitting a convex hull around the qubit locations in the barrier gate voltage space, we can estimate the volume of the region where qubits can be found. For this device, the volume of the convex hull is approximately $3.5\times10^{-4}$V$^3$, translating to a fraction of the safe ranges [$(2 \text{V})^3$] of about $4\times10^{-5}$. The space is further restricted by the plunger voltage location, which is a box of roughly $(10 \text{mV})^2$. Given a search space of $(300 \text{mV})^2$, this brings down the size of the volume to around $2\times10^{-7}$ as a fraction of the 5-dimensional gate voltage space. That is roughly equivalent to a needle in a $(2\text{m})^{3}$ haystack.

Once a qubit has been found, the algorithm allows for extensive characterisation. We can study 
$f_\text{Rabi}$ and the $g$-factor as a function of the barrier gate voltages (Fig.~\ref{fig:results}d). The resulting maps gives insights into qubit properties and can be extended to measure, e.g.~the Hahn-echo coherence time.%These measurements involve non-trivial automation, including the tracking of a transition, its read-out point, and $t_\text{burst}$ and would have been prohibitively expensive to take by a human.

% and 0.028\% of the space defined by each barrier's pinch-off. 
 
%We can gain insights into device physics by studying the locations where a qubit was found. If we fit a convex hull around the location in the barrier gate voltage space on where qubits were found, we get an estimation on how big the needle in the haystack is. In the given device, the convex hull has a volume of about $3.5\cdot10^{-4}$V$^3$. Expressed as a fraction of the safe ranges that is about 0.0043\%, as a fraction of the box spanned by the pinch off of each individual barrier that is 0.02756\%. The space is further restricted by the plunger voltage location, which is a box of roughly 10mV x 30 mV. Given a search space of 300mV x 300mV, this brings down the size of volume to around $1.45\cdot10^{-5}$\% as a fraction of the search space. That is roughly equivalent to a needle in a $1m^{3}$ hay stack. This analysis excludes the search for the Rabi and Larmor frequencies.

%The distribution of qubit locations in the barrier space can potentially accelerate the tuning of new devices with similar architecture.




\section*{Conclusions}
We have demonstrated fully automated tuning of spin qubits, progressing from a de-energised device to qubit control. Our algorithm autonomously achieved Rabi oscillations in 10 out of 13 trials. %, leveraging input parameters based on anticipated feature sizes and safety limits. 
Most tuning processes concluded within three days, with the primary speed constraint being the integration times required to perform DC transport measurements, which could be replaced by fast readout alternatives. 
Maps of the $g$-factor and $f_\text{Rabi}$ serve as evidence for the potential of this approach for high-throughput qubit characterisation.

%The algorithm reveals key requirements for achieving comprehensive automation:

%\paragraph{Robust and Efficient Framework} A system that seamlessly integrates all stages, equipped to handle dead-ends and capable of retracing steps when necessary.
 %\paragraph{Accurate Decision Algorithms} Algorithms must deliver high accuracy to minimize time lost on incorrect decisions. %An example is our use of neural networks for PSB detection in low-resolution scans, exemplifying this need. 
 %\paragraph{Optimized yet Flexible Optimization Algorithms}  The optimization algorithms are specifically tailored yet possess the flexibility to intelligently maneuver through the parameter space.

 
% Our work reveals key elements needed for full automation. Our approach required a robust and efficient framework designed to seamlessly integrate all stages, and handle dead-ends via a dynamic search tree when necessary, ensuring a continuous and smooth workflow. Additionally, accurate decision algorithms had to be integrated. These algorithms aim at significantly reducing tuning times. Our approach highlights the importance of algorithms that are both optimized and flexible. These are not just narrowly focused algorithms; they are specifically tailored yet exhibit inherent flexibility, allowing them to intelligently navigate through the device's parameter space. This combination of specificity and adaptability is crucial for the algorithm to effectively handle a wide range of device regimes.

The methodology is versatile and can be adapted for use with similar quantum devices, such as silicon FinFETs. The modular design of the algorithm allows for rapid adaptation to other architectures. For example, devices that use charge sensors and reflectometry for measurements would only require different signal-processing algorithms.

We anticipate that the mass tuning and characterization of qubits, facilitated by our fully autonomous tuning algorithm, will establish a productive feedback loop between measurement and fabrication processes. Wafer-scale, high-throughput characterisation of quantum devices, already feasible in early tuning stages, can mitigate device variability. This, in turn, improves the tuning process, bolstered by expanding datasets.

The first successful experiments on quantum computing with semiconductors were conducted nearly twenty years ago. 
%With this achievement of autonomous tuning, 
%We have now reached a notable point in our journey.
We have now confirmed the feasibility of fully automatic tuning of a semiconductor qubit. This breakthrough would allow us to move forward by leveraging the ability to mass characterise qubits to advance quantum circuit scalability in semiconductors.
%Each step since then has been made with respect for the complexity of the terrain and the knowledge of those who tread the path before us. As we reach a new milestone with autonomous tuning, we find ourselves at a higher vantage point, not at the summit, but at a significant ledge that offers a clearer view ahead. It's a moment to appreciate how far we've come, yet remain humbly aware of the climb that lies ahead in the ever-evolving landscape of quantum computing.
\bibliography{reference}

\newpage

\section*{Methods}
%The ‘Methods’ section is in the main text file, following the figure legends. This Methods section will appear in the PDF and in the full-text (HTML) version of the paper online, but will not appear in the printed issue. The Methods section should be written as concisely as possible but should contain all elements necessary to allow interpretation and replication of the results. As a guideline, the Methods section does not typically exceed 3,000 words. To increase reproducibility, authors are encouraged to deposit a detailed description of protocols used in their study in a protocol sharing platform of their choice. Nature Portfolio’s Protocol Exchange is a free and open service designed to help researchers share experimental know-how. Protocols deposited by the authors in Protocol Exchange will be linked to the online Methods section upon publication.

% currently: 3500 words

Here we provide details of the experimental set up, and algorithmic choices made in this study. We begin by describing the device used for our experiments. We then follow with a discussion of the intelligent computational approaches used in the algorithm. Finally, details of each stage are discussed. An overview of all the stages of the algorithm is given in Table \ref{tab:all-stages}.

Hyperparameters that are not explicitly given here can be found in the Supplementary Material.


\makeatletter\def\@currentlabel{Methods}\makeatother
\label{methods}

\section{The device, measurement apparatus and pulse sequence}
The device consists of a Ge/Si core/shell nanowire lying on top of nine bottom gates measured in a variable temperature insert (VTI) in a liquid helium bath with the sample mounted below the 1-K pot (base temperature 1.5 K). By applying positive voltages to the first five bottom gates from the left, an intrinsic hole gas inside the nanowire is depleted to form a hole DQD. An SEM image of a device similar to the one used here is shown in Fig.\ref{fig:device}. The device, measurement apparatus and pulse sequence are the same as used by Carballido \textit{et al.}~\cite{carballido2023qubit} and are described in detail in their work.


To amplify the measurements that rely on a microwave pulse, we applied a pulse-modulation by a lock-in amplifier at 87.777 Hz. The measurements therefore have an in-phase and out-of-phase component. We apply principal component analysis (PCA) to these measurements and project each measurement onto the principal axis. We further offset the measurements such that they are strictly positive. Measurements that are obtained this way are marked with $I_\text{LI}$, as opposed to currents that were measured conventionally which are marked with $|I|$.%$|\tilde{I}_\text{SD}|$.




\section{Techniques used in the algorithm}
% -------- Nathan
%In order to achieve a
Useful automation of tuning from a de-energised device to identification of Rabi oscillations requires an algorithm that can adapt to different data capture regimes, and be transferred to other, similar devices. To achieve this, we have made extensive use of intelligent, adaptive and data-driven subroutines. Nowadays, there is a plethora of such techniques to choose from, and in order to choose the right technique to apply to each stage of the algorithm, we considered:
\begin{itemize}
    \item the need for expert labelled training data, which was not always possible or realistic to source;
    \item the need of being efficient both in the total number of measurements taken during a stage, and in the resources needed for computing decisions about which measurements to take;
    \item the minimal accuracy needed in each stage for the whole algorithm to be able to achieve its overall goal of identifying operating parameters for a qubit.
\end{itemize}
To address the above considerations across the many stages of the algorithm, a non-exhaustive list of techniques we have found useful to employ includes Gaussian process (GP) inference, convolutional neural networks (CNNs), unsupervised computer vision (CV) and computational geometry techniques, and Bayesian optimisation (BO). We now briefly introduce these, highlighting their strengths and weaknesses.

GPs are a popular form of non-parametric Bayesian inference \cite{Rasmussen2005GaussianPF}. They can be thought of as a method for doing principled Bayesian inference over a space of functions. GPs can be tailored to any specific domain or problem by making a choice of the so-called kernel (or covariance) function, a part of this model which describes prior knowledge about the possible space of functions in which inference is to occur. This choice can allow practitioners to encode important domain knowledge before capturing any data, such as specifying knowledge of periodicities, symmetries or the expected degree of smoothness of the underlying process that is being observed. This constitutes the main strength of GP modelling, often enabling highly data-efficient inference. However, both model fitting and model prediction can be computationally intensive, typically growing cubically \cite{Rasmussen2005GaussianPF} in the number of observed data points.

Over the past two decades, CNN architectures have proved to be go-to models for solving computer vision tasks. Their strengths lie in their adaptability across different computer vision tasks, their robustness in the face of unknown noise, and their computational efficiency at training time. Their weakness lies in always requiring substantial amounts of training data. In this work, we use some standard architectures, such as ResNet \cite{He2015DeepRL} as tools for extracting properties from or making assessments of stability diagrams. Where we have applied them, training data has been either generated by a sufficiently good simulator, or gathered from this or similar devices and then labelled by an expert.

Often, the use of CNNs is neither required nor appropriate for the particular computer vision task at hand. In particular, it has been of crucial importance to a number of stages through the algorithm to be able to automatically locate and segment bias triangles within stability diagrams using a coordinate-wise approach. To achieve this we have employed a number of unsupervised computer vision techniques that can mitigate noise in, and localize features of the geometric figures present in stability diagrams. Whereas CNNs would require large amounts of labelled training data to achieve this result, the requirements can be met by computer vision techniques that need no training data, and require only a few hyperparameter choices to be made. All together we have called this a bias triangle segmentation framework, and it is described in \cite{kotzagiannidis2023bias}, where the specific application to PSB detection is also detailed.

Bayesian optimisation \cite{Shahriari2016TakingTH} is a general, iterative approach to black-box function optimisation. At each iteration, it constructs a surrogate model of the function being approximated using the data already gathered, and uses this surrogate model to efficiently compute the next most informative location from which to sample the unknown function. In order to apply this technique one must specify a score function to optimise and a parameter space over which the search for an optimum is conducted. The choice of the surrogate model is also influential in the accuracy, efficiency and reliability achieved using this method. In this work we have made consistent use of GP surrogate models using a Matern 5/2 kernel.

\section{Stages of the algorithm}

\subsection{Define DQD}
\subsubsection{Hypersurface building}
% ---------- JONAS

As a first step, the algorithm determines a current that it considers to be pinched off by ramping to the high end of the safe ranges. We take repeated current measurements there to characterise the noise floor. From the noise floor we compute a pinch off current. 

Next, we sample several points within the safe ranges using a Sobol sequence for quasi-random locations. The points are used to define rays from the origin that are then investigated for pinch off. To avoid overloading the current amplifier, we search for pinch off from the origin towards the upper end of the safety ranges with a low bias voltage. Once pinch off is found, we retrace with a higher bias voltage to confirm the exact pinch off location. 

Finally, we use this data to construct the hypersurface model as outlined in the main text.

% 

% Then a number of points within the safe ranges are sampled using quasi-random locations via a Sobol sequence. The points are used to define rays from the origin that are then investigated for pinch off. To avoid overloading the current amplifier, we search for pinch off from the origin towards the upper end of the safety ranges with a low bias voltage. Once pinch off is found, we retrace with a higher bias voltage to confirm the pinch off. 

% The hypersurface model is then built as described in the main text.


\subsubsection{Double dot detection}
% ---------- JONAS
The previous stage defines a region within which we can look for a DQD potential. We sample quasi-random points via a Sobol sequence for investigation. For each point, we vary both plunger voltages simultaneously and measure the current, following the method described by Moon \textit{et al.}~\cite{moon2020machine}. We use the random forest classifier developed by Severin \textit{et al.}~\cite{severin2021cross} to check for the presence of Coulomb peaks. If Coulomb peaks are found, we then measure a stability diagram. This diagram is analyzed with a neural network to detect features of the DQD. The neural network was trained on data from a variety of devices, mainly from the data gathered by Moon \textit{et al.}~\cite{moon2020machine} and Severin \textit{et al.}~\cite{severin2021cross}, and additional data from a nanowire device different from the one used in this work. In total, there were 4,611 stability diagrams of which 726 showed double dot features.

%The previous stage defines a region within which we can look for a DQD potential. We sample quasi-random points via a sobol sequence for investigation. At each point that is investigated we first take a tracee varying both plunger voltages equally and recording the current, as also described by Moon \textit{et al.}~\cite{moon2020machine}. We use the exact same classifier, a random forest, developed by Severin \textit{et al.}~\cite{severin2021cross} to decide whether Coloumb peaks are present. If they are, a stability diagram is taken. It is analyzed by a neural network for DQD features. 


\subsection{Tune barriers}
\subsubsection{Barrier optimisation}
Upon formation of separated pairs of bias triangles, we perform coordinate-wise segmentation and polygon fitting (see Sect.~\ref{app:segmentation} %Sect. III. B. 
for more details, \cite{kotzagiannidis2023bias}) in order to facilitate their tracking and feature extraction throughout the remainder of the tuning pipeline.

The segmentation and shape extraction enable the assessment of the current intensity difference between the base line and gap formed between the base and first excited state line. By quantifying this intensity difference in a base separation score, we can employ a Bayesian optimisation framework which seeks to maximize the intensity difference, as a promising indicator for detecting viable candidates for PSB.

Each pair of bias triangles should present a base well separated from the main body. The wider the separation, the better the protection of the ground state and the more likely it is that we are in the presence of a qubit. The separation score is computed by averaging the current along the detuning axis, see the two one-dimensional traces in Fig.~\ref{fig:algo_illustration} b-ii, and computing the ratio of the intensity between the peaks and the lowest point in the valley between them. In the case of multiple triangles, the highest separation is used as score.
% JS: I excluded this from the manuscript as I believe this functionality wasn't active in the runs that are in this paper. I am not sure why, but it also seems to have had no or little effect as there weren't many/any encounters of co-tunelling in those runs.
% Another aspect of barrier optimisation is to steer away from areas in parameter space where co-tunneling is present. From a visual perspective, co-tunneling %is a leakage of electrons that 
% can be noticed by lines, parallel to the axes, connecting the bias triangles. In case co-tunneling lines are detected, the parameter space for the Bayesian Optimiser is trimmed. We trim the barrier voltage dimension that is associated with the plunger voltage along which the co-tunneling line exists, i.e.~if there are co-tunneling lines along the left (right) plunger voltage axis, we consider the current left (right) barrier voltage setting to be the new lower limit. % along the relative axis, considering only barrier values that are above the one at the current location.

Certain potential landscapes can lead to situations in which charge configurations are affected by charge switch noise.  
%In our analysis, we encountered a challenge with certain candidate triangles exhibiting high levels of noise, likely due to internal charge fluctuations. We refer to these anomalies as 'switch-y' triangles. 
Since these potentials are unlikely to be used as a qubit and the resulting bias triangles can skew our base separation scoring, we excluded them by leveraging a neural network classifier. This classifier was trained to distinguish between normal bias triangles and ones that are affected by charge switch noise, as illustrated in Fig.~\ref{fig:switch_illustration}. The training dataset for this classifier was obtained as follows: initially, potential bias triangles were identified using our segmentation routine. Subsequently, we hand-labeled 2,302 of these (1,539 samples showed no switch noise) to create a robust training set. The classifier itself was then obtained by fine-tuning a ResNet-based architecture with this dataset. 

Once the voltage space has been explored through BO we have a clear understanding of the landscape, as in Fig.~\ref{fig:algo_illustration} b-ii. The measurements in this optimisation were obtained using an efficient measurement algorithm, see Supplementary Materials for details. We sample the most promising regions again without the efficient measurement algorithm and analyse them as described in the next section. %To speed up the full procedure it's important to select and prioritise the plunger windows with the highest scores.

%\hl{2302 samples, 1539 negatives, 91 some switches}

\subsubsection{Plunger window selection}
Given a sampled stability diagram containing bias triangles, the aim is to select the region that contains as many bias triangles with scores as high as possible, no areas with current that is too high, and as few switches as possible as depicted in Fig.~\ref{fig:algo_illustration} b-iii. High current bias triangles are unlikely to be able to be used for qubit operations. This is a heuristic and we set a conservative threshold of 200 pA. To ease the downstream steps, the region should be a rectangular window. Through an iterative approach, starting from the smallest bounding boxes containing each single pair of bias triangles, larger windows are constructed by merging the existing ones in case they satisfy the conditions about switch absence and low currents. For the switches absence we used a soft constraint, allowing for bias triangles affected by switch noise in case their total area was less than 25\% of the area covered by all triangles in the window. The algorithm complexity scales exponentially with respect to the number of triangles and some heuristics have been leveraged to reduce substantially complexity and therefore execution time. In particular, at each iteration, only the top 100 bounding boxes by the number of contained triangles without switches were kept, to ensure a manageable upper limit on the number of possible merges. The routine halts when no further merges are possible.  
Once the plunger windows have been selected they are ranked by highest separation score. % and sampled again with higher resolution to enable the PSB search.


\subsection{Find PSB}
\subsubsection{Wide shot PSB detection}
% ---------- Jonas
To identify each bias triangle's location, we first leverage the fact that they sit on a honeycomb or skewed rectangle pattern. We use autocorrelation on the stability diagram to identify this pattern. The largest two peaks in the autocorrelation help us establish a vector that spans this pattern of skewed rectangles. To fix the pattern in place, we employ a blob detection algorithm, using the first blob it identifies. This helps us accurately overlay the skewed rectangle pattern and estimate the locations of the bias triangles (Fig.~\ref{fig:autocorrelation}).

Next, we extract these bias triangles using the identified locations, with side lengths informed by the pattern dimensions. These extracted bias triangles are then input into a neural network for further analysis. We used autonomously gathered data that was taken during the initial development phase. In total, we used 626 pairs of bias triangles taken from 70 stability diagrams. 55 of the pairs of bias triangles showed PSB. For more detailed information on this procedure, see Schuff \textit{et al.}~\cite{schuff2023identifying}.

% We first need to find the location of each bias triangle. To facilitate this we use the fact the they are placed on a honeycomb patter, or more simple, a pattern of skewed rectangles at their corners. We take the autocorrelation of the stability diagram which finds this patter. The first two maxima in the autocorrelation defines a spanning vector for the skewed rectangle pattern. To anchor this pattern we use a blob detection algorithm and use the first blob it finds, then overlay the skewed pattern on top to get estimations of the location of the bias triangles. 

% We cut out the bias triangles using those locations. for the sidelength we use information from the skewed pattern. The cutouts are then fed to a neural network, see \cite{schuff2023identifying} for details.




%\hl{TODO: 
% - Details on training data for PSB detection.}
%(626 samples, from 70 scans, with 55 positives)


\subsubsection{Re-centering and high resolution PSB detection}
\label{app:segmentation}
% ---------- Madeleine
In an effort to filter the previously detected 
candidates for PSB and eliminate false positives, a second set of higher resolution measurements is performed. For that purpose, a dedicated low resolution stability diagram of the candidate bias triangles is taken and used to update the plunger voltage extent based on the detected contours, effectively performing a re-centering. With the updated voltage extent, high resolution stability diagrams with $B = 0 $ T and with $B=0.1$ T are taken.\\
\\
A second sub-stage of PSB-classification is applied through a segmentation-based detection and feature extraction framework, which facilitates the coordinate-wise quantification of geometric and physical properties of bias triangles \cite{kotzagiannidis2023bias}.
In particular, given the high-resolution stability diagram with $B=0.1$ T, this framework fits minimum-edge polygons to the detected contours of bias triangle pairs by utilizing a relaxed extension of the Ramer-Douglas-Peucker algorithm \cite{kotzagiannidis2023bias}.
Once the segmented shape mask is identified, further geometric properties such as the base and excited state lines can be automatically extracted solely based on the prior knowledge of the bias voltage sign, which predicts the direction in which bias triangles point.\\
\\
For the identification of PSB, an analytical classifier based on the above framework was devised \cite{kotzagiannidis2023bias}. PSB expresses itself as a suppressed base line of the bias triangles at $B=0$ T. At $B>0$ T, there is a leakage current at the base line. The routine extracts the segment enclosing the base and a prominent excited state line on the stability diagram with leakage current ($B=0.1$ T). Subsequently, the average pixel intensity of the segment normalised by the intensity of the entire pair of bias triangles is computed. By superimposing the detected segment on the scan with blocked current ($B=0$ T), normalised intensity values are compared and, if their difference exceeds a specified threshold, the charge transition is identified as positive for PSB.\\
\\
Based on the segmented bias triangle shape mask, further geometrical properties can be automatically extracted, which enables the tuning of bias triangle features in stage 2.
\\
The detuning axis, utilized for the Danon gap measurement, is automatically extracted by identifying the bias triangles base midpoints and tips and computing the lines between them.



\subsubsection{Danon gap check}
\label{app:danon_gap_check}
% ---------- Jonas to add in some physics descriptions (see the square brackets)
As a further filter for possible candidates, we check to magnetic field dependence of the leakage current at the base of the bias triangles in a different way. As a function of the applied magnetic field $B$, we expect the leakage current to be minimal at $B=0$ T and higher away from this point. We call this the Danon gap \cite{danon2009pauli}. A current measurement of the detuning line while varying the magnetic field gives us a two-dimensional input (Fig.~\ref{fig:danon_gap}), which we can analyse as follows: Ignoring the noise signal, the current is roughly constant along the magnetic field axis, whereas the detuning line axis is information-rich: away from the Danon gap there are two local extrema (to one side the noise floor outside the bias triangles, to the other side the gap due to singlet-triplet energy splitting) whilst the Danon gap region is characterised by a monotonic behaviour, with roughly a constant value. 
\\
To detect the presence of the Danon gap, the current $I$ is firstly processed with a Gaussian filter, to smooth out the noise, and then the absolute slopes along the detuning line axis are integrated $g(B):= \sum_{\varepsilon}{\left|\frac{\partial \tilde{I}(\varepsilon,B)}{\partial \varepsilon}\right|}$, where the derivative is the discrete derivative along the detuning line axis. The function $g$ is minimised in the areas where the smoothed signal $\tilde{I}$ shows a constant value. We show the normalised function $\bar{g} = \frac{g}{|\varepsilon|}$ in Fig.~\ref{fig:danon_gap}. To detect the presence of the Danon gap from $g$ two tunable hyperparameters are used, validating the depth and width of the basin of the global minimum of $g$: in case the basin is not prominent enough there is no Danon gap. As the last check, the location of the minima has to be in proximity of zero magnetic field.
\\
%In case all the checks are satisfied the magnetic field location that minimises $g$ is returned, otherwise the candidate is discarded.

\subsection{Find readout}
\subsubsection{Tracking \& entropy optimisation} % TODO: Split out tracking as a separate subsection
% ---------- Madeleine
In subsequent steps, we apply a pulse sequence to the right plunger electrode. As it is a two-stage pulse, the bias triangles will have a `shadow' in the stability diagram. We need to identify the original bias triangles and find a suitable region where we can expect to find qubit readout. %, as the position of the bias triangle may change and split triangles (i.e. a mirroring effect which leads to the doubling of bias triangle pairs within the scan) occur as a result of pulsing, we track the segmented triangle by performing template matching. 
In light of resulting shape distortions and further degrading effects to the measurement quality, we opt for template matching as opposed to performing re-segmentation for bias triangle tracking in order to ensure robustness.\\
\\
The relative direction in which the shadow bias triangles appear with respect to the original one is known in advance due to the applied pulse shape. This is incorporated into the shape matching approach as the cardinal direction to uniquely identify and track the triangles.
\\
We perform shape matching by comparing the edge map of a stability diagram prior to pulsing, functioning as the template, to the edge map of a subsequent stability diagram with pulsing, functioning as the source for current information. Further, we extract the segmented shape mask from the template.
The method slides the template over the source edge map, thereby comparing the template with individual patches of the stability diagram with pulsing, and returns a result matrix (of the same size as the source) whose individual entries quantify the similarity with the template patch. The employed similarity metric is the normalized correlation coefficient and the patch with maximum
correlation is selected. Once the appropriate patch has been identified, the initial segmentation mask of the stability diagram without pulsing is mapped to the stability diagram with pulsing and used for subsequent processing. 
\\
In order to identify the optimal readout spot, we extract the segment enclosing the base and prominent excited state lines on the obtained segmented mask of bias triangles with pulsing, and perform Bayesian optimisation of a readout quality score over four parameters: the constrained two-dimensional plunger gate voltage space, frequency of the driving pulse $f_\text{MW}$ and burst time $t_\text{burst}$.
\\
Optimal readout candidates are those which meet the resonance conditions of the qubit. If they are met, there is a leakage current that we record using the lock-in amplifier. For a given burst time $t_\text{burst}$ (relating to the Rabi frequency $f_\text{Rabi}$) and a given frequency of the driving pulse $f_\text{MW}$ (relating to the $g$-factor), the leakage is characterized as a peak in leakage current for a certain magnetic field $B$. Thus, for the readout optimisation, we use measure the current with varying magnetic fields. Instead of applying PCA, as explained above, we use the L2 norm of the in-phase and out-of-phase components to retrieve a one-dimensional trace $l(B)$. This guarantees peaks to be higher than the background, as opposed to processing with PCA, which can lead to dips rather than peaks.

To quantify the sharpness of these peaks%(readout quality score)
, we developed a score based on the Shannon entropy $H = -\sum_B \left[l(B) \log(l(B)\right]$ of the trace. For the calculation of the entropy of the score, we first subtract the median and then clip values at zero. This particular pre-processing turns the trace into something more akin to a distribution and enhances the robustness of our score, making it less susceptible to potential noise disturbances in the trace. This method results in a smooth score landscape suitable for Bayesian optimisation.

\subsubsection{Resonance confirmation}
This verification step acts as a final filter and the last stages are all executed once a candidate passes this filter. The previous stage sends a candidate with a suspected resonance condition. The stage re-measures the leakage current as a function of the magnetic field. If the resonance condition was truly found, a peak should appear at the same magnetic field again. Should a peak with a specified prominence at this magnetic field within a set margin of error be detected, the resonance condition is considered confirmed and all downstream measurements are executed.
We note that a noisy candidate might pass this stage. Repeating the verification step can reduce such occurrences.

%This step revisits and verifies the final data from the previous stage. If the EDSR peak is consistent, it will be observed again and identified using scipy. The earlier stage indicates a potential magnetic field. Should a peak be detected with a specified prominence and it corresponds to this magnetic field within a set margin of error, the presence of EDSR is confirmed. This is the final validation step, and subsequent processes are initiated only after a candidate clears this phase. Note that due to inherent variability, some noisy candidates may progress; however, repeating this verification step can reduce such occurrences.

%This step simply retakes the final data from the previous step. If the EDSR peak is reproducible, we should see it again and be able to find the peak using scipy. The previous stage communicates a suspected magnetic field. If any peak that is found with a given prominence is at this magnetic field (within a certain margin of error) we confirm the presence of EDSR.  This step is the last filtering stage and the last stages are all executed once a candidate passes this stage. We note that a noisy candidate might therefore pass this stage. This could be addressed by repeating this check a number of times.

\subsubsection{Qubit measurements}
% ---------- Jonas

% For this measurement we vary the magnetic field and the burst duration. The characteristic Rabi chevron can be analysed by considering the frequency spectrum for each magnetic field. The frequency should have a minimum at the magnetic field that meets the resonance condition of the qubit. The amplitude should also be maximal there due to decoherence for off-resonant driving. 

%

Once a resonance condition is found, we vary the magnetic field and the burst duration. The characteristic Rabi chevron can be analysed by considering the frequency spectrum for each magnetic field. The frequency should have a minimum at the magnetic field that meets the resonance condition of the qubit. The amplitude should also be maximal there due to decoherence for off-resonant driving.
We can therefore simply look for the maximum amplitude in the Fourier transformed Rabi chevron (Fig.~\ref{fig:chevron_analysis}). This information will give us the precise resonance conditions for the last step, repeated measurements of Rabi oscillations on resonance.

\section{Characterisation}

The maps in Fig.~\ref{fig:results} were generated using automated measurements. Initially, upon identifying a qubit, we record its readout spot, $g$-factor, and $f_\text{Rabi}$. We then alter the confinement potential by slightly adjusting the barrier gate voltages. This adjustment may shift the bias triangles, consequently moving the readout spot, $g$-factor, and $f_\text{Rabi}$. Our method involves tracing these transitions to locate the readout spot in its new position. At this new location, we conduct an EDSR check scan. Any changes in the peak's location inform us about variations in the $g$-factor. Furthermore, measuring Rabi oscillations at this point helps update our understanding of $f_\text{Rabi}$.

As we progressively deviate from the initial measurement point, we utilize our closest prior qubit data to infer the properties at the new location. This step is crucial as a shift in the $g$-factor necessitates modifying the magnetic field range, while a change in $f_\text{Rabi}$ requires adjusting the $t_\text{burst}$ duration for the EDSR check to accurately detect resonances.

% Determining $f_\text{Rabi}$ involves fitting Rabi oscillations, a process more susceptible to noise compared to the simpler peak finding method used for the g-factor. Hence, the data points used to map $f_\text{Rabi}$ are a subset of those employed for the g-factor map.


% were taken with the help of automated measurements. Once a qubit has been identified, we can note the readout spot, the $g$ factor and $f_\text{Rabi}$. We can then vary the confinement potential by slightly changing the barrier gate voltages. This might move the bias triangles, and with it the readout spot, the $g$-factor and $f_\text{Rabi}$.
% We can track where the transition moved, find the readout spot in the new position, and perform an EDSR check scan at the new readout spot. The location of the peak updates our knowledge of $g$.  A subsequent measurement of Rabi oscillations updates our knowledge of $f_\text{Rabi}$.

% As we move further away from the initial point, we can use the knowledge of the qubit at the location closest to a new location to guess the new properties. This is important because a shift in the $g$-factor means that the window in magnetic field may need to be adapted and a change in $f_\text{Rabi}$ means that the $t_\text{burst}$ for the EDSR check needs to be updated to see the resonance. 

% The determination of $f_\text{Rabi}$ involves fitting the Rabi oscillations, which is more prone to noise than the simple peak finding for the $g$-factor. Therefore, the points for the $f_\text{Rabi}$ map is a subset of the points for the $g$-factor.


\section*{Acknowledgements}

This work was supported by the European Research Council (grant agreement 948932), the Royal Society (URF-R1-191150), Innovate UK project AutoQT (grant number 1004359), NCCR SPIN of the Swiss NSF, Swiss Nanoscience Institute (SNI), the EU H2020 European Microkelvin Platform EMP (grant no. 824109), FET TOPSQUAD (grant no. 862046), and FETFLAG QLSI (grant no. 951852).
% The research leading to these results has received funding from the European Union's Horizon 2020 Research and Innovation \textit{Programme European Microkelvin Platform (EMP)}.
J.S.~acknowledges financial support from the EPSRC (grant number R72976/CN001).

We want to thank Andrew Briggs, Georgios Katsaros, Dominic Lennon and Leon Camenzind for helpful discussions.

\section*{Author Contributions}

% J.S.~performed the experiments with M.J.C.'s guidance and help from T.P.~in D.M.Z.'s lab. M.J.C. fabricated the device. 
% %N.A.( and ...?)~conceived of the project. J.S. and M.J.C.~planned the experiments. 
% J.S.~developed the algorithm, in particular the modular framework and the overall algorithm flow. J.S., M.J.C., D.C., B.v.S., N.K., M.K., M.C., J.R., and J.C.C. developed routines for the stages. J.S.~lost his marbles. J.S. analysed the data. N.A. conceived of the project. J.S.~wrote the manuscript with inputs from all authors.

% ----- Suggested rewording from Nathan:
J.S.~developed the algorithm, in particular the modular framework and the overall algorithm flow.
J.S.~performed the experiments and analysed the results with M.J.C.'s guidance and help from T.P.~and R.S.E.~in D.M.Z.'s lab. M.J.C.,~S.S.~and P.C.K.~fabricated the device. J.S., M.J.C., J.C.C., M.K., M.C., J.R., N.K., D.C., B.v.S.~and B.S.~developed the routines for the various stages of the algorithm, including analysing and interpreting data, making algorithm design choices, and writing the software used to run and record the experiments.
% J.S.~lost his marbles.
J.C.C., M.K., M.C., J.R., and N.K. made substantial independent contributions to the Methods and Supplementary Materials sections.
J.S.~wrote the manuscript with inputs from all authors.
N.A.~conceived of the project.

\section*{Data and Code Availability}
The data and code will be made available upon final publication.



%\printbibliography

%\section*{Methods}

%\include{appendix}

\newpage

\appendix

\clearpage


\section*{Extended Data}\label{app:...}



\begin{figure}[!htbp]
\centering
  \includegraphics[width=.66\linewidth]{figures/device.pdf}

  \justifiedcaption{ \textbf{Device.}  False color micrograph of a nanowire device similar to the one used in this work. The Ge/Si nanowire is colored in yellow.}
  \label{fig:device}
\end{figure}

\FloatBarrier
\begin{figure}[!htbp]
\centering
  \includegraphics[width=1\linewidth]{figures/autocorr_demo.pdf}

  \justifiedcaption{ \textbf{Bias triangle locations via auto-correlation.} A stability diagram (top left) is processed using its auto-correlation (top right). Within the auto-correlation, we can find the highest values to span a grid of skewed rectangles. The extracted information is used to locate bias triangles in the original stability diagram (bottom).
  }
  \label{fig:autocorrelation}
\end{figure}
\FloatBarrier

\begin{figure}[htbp]
\centering
  \includegraphics[width=1\linewidth]{figures/switch_illustration.pdf}

  \justifiedcaption{ \textbf{Effect of charge switch noise.} Stability diagrams can be affected by charge switches. Their effect can be seen in the left column. For comparison, the right column is unaffected by these charge switches.}
  \label{fig:switch_illustration}
\end{figure}

\FloatBarrier

\begin{figure}[!htbp]
\centering
  \includegraphics[width=1\linewidth]{figures/danon_gap.pdf}

  \justifiedcaption{ \textbf{Danon gap check.} As final check to confirm the presence of PSB, the algorithm takes measurements of the detuning line $\varepsilon$ (marked in the left panel) as a function of the magnetic field $B$ (middle). The measurement is analysed, as described in \ref{app:danon_gap_check}, by first computing the averaged sum of absolute derivatives $\bar{g}$ (right). If a dip is present in $\bar{g}$ close to $B=0$ T, PSB is confirmed.}
  \label{fig:danon_gap}
\end{figure}

\begin{figure}[!htbp]
\centering
  \includegraphics[width=1\linewidth]{figures/chevron_analysis.pdf}

  \justifiedcaption{ \textbf{Rabi chevron analysis.} A qubit that is driven close to the resonance condition exhibits so-called Rabi chevrons, see left column for examples (top: simulation, bottom: experimental data). To find the resonance frequency, we analyse the frequency spectrum for each magnetic field (which controls the detuning from resonance). The frequencies have a maximum amplitude and a minimal point at the resonance condition.}
  \label{fig:chevron_analysis}
\end{figure}

\begin{table*}[htbp]


  \centering
    \begin{tabularx}{\textwidth}{l||X|X|X}
            Stage                    & Description                                                                        & Techniques used                                                             & Candidate information                                             \\
\toprule
\toprule
\textbf{Stage 1:} Define DQD \\
\textbf{a,} Hypersurface building  & Building a model of the surface that separates pinch-off from conducting  & Gaussian processes & Upper and lower bounds of barrier voltages  \\
\textbf{b,} Double dot detection  & Identifying Coulomb peaks and double dot signatures & Random forests and neural networks & Corrected lower bound of barrier voltages \\
                  
    \midrule
                
\textbf{Stage 2:} Tune Barriers\\
\textbf{a,} Barrier optimisation& Search over the barrier voltage space for ideal settings & Bayesian optimisation, computer vision, neural networks& Promising barrier voltage location \\
\textbf{b,} Plunger window selection & Determine a window for plunger voltages & Computer vision, neural networks& Barrier voltage location and wide plunger voltage range \\

    \midrule
            
\textbf{Stage 3:}   Find PSB  \\
\textbf{a,} Wide shot PSB detection& Identify locations of transitions with PSB & Neural networks, computer vision & Narrow plunger voltage range \\
\textbf{b,} Re-centering & Get precise plunger voltage window & Computer vision & Corrected narrow plunger voltage range \\
\textbf{c,} High res.~PSB detection & Confirm PSB with high resolution measurement & Computer vision & Narrow plunger voltage range, link to high res.~measurement, detuning line definition\\
\textbf{d,} Danon gap check & Confirm PSB by measuring detuning line as a function of magnetic field & Computer vision & Narrow plunger voltage range, link to high res.~measurement \\

    \midrule
    
\textbf{Stage 4:} Find Readout\\
\textbf{a,} Entropy optimisation & Find readout spot, $g$-factor and Rabi frequency by optimisation of an entropy score & Bayesian optimisation, computer vision & Precise plunger voltage locations, magnetic field, drive frequency and burst time \\
\textbf{b,} Resonance confirmation & Confirm resonance from previous stage/filter out noise& Peak finding & Passed on from previous \\
\textbf{c,} Spectroscopy& Measurement of current while varying $t_\text{burst}$ and $f_\text{MW}$ for documentation& -& Passed on from previous\\
\textbf{d,} Rabi chevron& Measuring Rabi oscillations close to the resonance condition & Frequency analysis& Corrected magnetic field for resonance condition\\
\textbf{e,} Rabi oscillations& Take repeated Rabi oscillations on resonance & - & - \\                                                 
\bottomrule
\end{tabularx}
\justifiedtablecaption{\textbf{List of all stages.} We list all stages and sub-stages with a short description, a rough overview of what techniques were used and what the information is passed downstream for a candidate from each stage. Besides information on the parameters that are directly needed to operate a qubit, the stages also pass down meta-information that other stages might need to use, e.g.~the high resolution stability diagram of Stage 3c is needed in Stage 4a for template matching.}
\label{tab:all-stages}
\end{table*}%

% \begin{figure}[ht]
% \centering
%   \includegraphics[width=0.9\linewidth]{figures/tuning_times_locations.pdf}

%   \justifiedcaption{ \textbf{Stage structure.}  Common structure of each stage}
%   \label{fig:device}
% \end{figure}



